On the dynamics of spicules and mass flows in the solar atmosphere

Popular scientific summary -- The atmosphere of the Sun is envisioned as composed of inherently complex, non-homogeneous, and dynamic layers. A detailed understanding of the physical processes involved in these layers is still lacking. For example, it is largely unknown why the outermost layer of the Sun's atmosphere (the solar corona) is so much hotter than the photosphere by millions of degrees. Astrophysicists think that the layer sandwiched between the photosphere and the corona, known as the interface region, may hold the key to a better understanding of the nature of this enigma. With the help of coordinated high-resolution, ground- and space-based observations from the Swedish 1-m Solar Telescope (SST) on La Palma, Spain, and NASA's Interface Region Imaging Spectrograph (IRIS) and Solar Dynamics Observatory (SDO), along with the support from an advanced numerical simulation, I aim to unlock some of the mysteries surrounding the dynamics of the interface region with a focus on small-scale jets, known as "spicules". Spicules are found almost everywhere on the Sun's surface and at any given moment there can be as many as 10 million of them rapidly shooting outwards. They are often found to be heated beyond chromospheric temperatures and appear in the transition region and (even) coronal passbands. Because of their "omnipresence", it is suggested that they play a major role in energizing the outer atmospheric layers of the Sun. This thesis focuses on the physical characteristics and dynamics of spicules, along with their role in mass-balance and heating of the solar atmosphere.

==> sections/paperI.tex <==
\author
{
    Souvik~Bose
    \and
    Vasco~M.J.~Henriques
    \and
    Jayant~Joshi
    \and
    Luc~Rouppe~van~der~Voort
}
\title{Characterization and formation of on-disk spicules in the Ca~II~K and Mg~II~k spectral lines}
\metadata{A\&A 631, L5 (2019), DOI: \url{https://doi.org/10.1051/0004-6361/201936617}}
\maketitle
\label{pap:Paper1}

\includearticle{sections/Paper1}
% \includearticle{sections/a4paper}

==> sections/paperII.tex <==
\author
{
    Souvik~Bose
    \and
    Jayant~Joshi
    \and
    Vasco~M.J.~Henriques
    \and
    Luc~Rouppe~van~der~Voort
}
\title{Spicules and downflows in the solar chromosphere}
\metadata{A\&A 647, A147 (2021), DOI: \url{https://doi.org/10.1051/0004-6361/202040014}}
\maketitle
\label{pap:Paper2}

\includearticle{sections/Paper2}
% \includearticle{sections/a4paper}

==> sections/paperIII.tex <==
\author
{
    Souvik~Bose
    \and
    Luc~Rouppe~van~der~Voort
    \and
    Jayant~Joshi
    \and
    Vasco~M.J.~Henriques
    \and
    Daniel Nobr\'egra-Siverio
    \and
    Juan Mart\'inez-Sykora
    \and
    Bart~De~Pontieu
}
\title{Evidence of multithermal nature of spicular downflows}
\subtitle{Impact on solar atmospheric heating}
\metadata{Forthcoming article in \textit{Astronomy \& Astrophysics}\\ DOI: \url{https://doi.org/10.1051/0004-6361/202141404}}
\maketitle
\label{pap:Paper3}

\includearticle{sections/Paper3}
% \includearticle{sections/a4paper}
